Reaching Consensus in the Byzantine Empire: A Comprehensive Review of BFT Consensus Algorithms

Byzantine fault-tolerant (BFT) consensus algorithms are at the core of providing safety and liveness guarantees for distributed systems that must operate in the presence of arbitrary failures. Recently, numerous new BFT algorithms have been proposed, not least due to the traction blockchain technologies have garnered in the search for consensus solutions that offer high throughput, low latency, and robust system designs. In this paper, we conduct a systematic survey of selected and distinguished BFT algorithms that have received extensive attention in academia and industry alike. We perform a qualitative comparison among all algorithms we review considering message and time complexities. Furthermore, we decompose each consensus algorithm into its constituent subprotocols for replication and view change backed by intuitive figures to illustrate the message-passing pattern. We also elaborate on the strengths and weaknesses of each algorithm as compared to the state-of-the-art approaches.

==> protocols/epaxos-fei.tex <==

\subsection{EPaxos: There Is More Consensus in Egalitarian Parliaments}

\subsubsection{System model and service properties}
 
Egalitarian Paxos (EPaxos) is a leaderless non-Byzantine fault tolerant consensus protocol that tolerates $f$ crashed failures with at least $2f + 1$ servers in total~\cite{moraru2013there}. EPaxos provides higher availability and higher performance by eliminating the designated primary(leader) node in the system: workload from clients is distributed based on the geographical features of replica instead of flowing into a single leader node. Therefore, EPaxos avoids the system interruption caused by a leader failure and leader re-election compared to its predecessors, Muliti-Paxos~\cite{lamport1998part, lamport2001paxos}, Mencius~\cite{barcelona2008mencius}, Fast Paxos \cite{lamport2006fast}, Generalized Paxos~\cite{lamport2005generalized}, etc. The manner of location-based workload distribution also enables Epaxos to reduce the message latency and improve the system throughput. In addition, Epaxos provides a \textit{fast path} that allows a node to commit a message after only one round of message communication within a quorum of $f + \lfloor \frac{f+1}{2} \rfloor$ nodes (with proof in~\cite{moraru2013proof}), including the node receiving the message and initiating the commit request. Such node is called \textit{command leader} in EPaxos (\textit{message primary} in this paper). EPaxos has message transmission cost of $O(n)$ for each committed message. 


\subsubsection{ Consensus for regular operations (fast path and slow path)}

\begin{figure*}[h]

    \begin{subfigure}{0.43\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/epaxos-fast-path.pdf}
        \caption{Fast Path in EPaxos.}
        \label{fig:epaxos-fast-path}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.55\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/epaxos-slow-path.pdf}
        \caption{Slow Path in EPaxos.}
        \label{fig:epaxos-slow-path}
    \end{subfigure}
    \caption{The message-passing workflow in Epaxos with $n=5$, $f=2$.}
    \label{fig:sbft}
    

\end{figure*}

EPaxos separates \textit{committing} and \textit{executing} a command message into two actions. Clients only know whether a command finished its execution or not by sending a \msgtype{read} request \msg{Read, objectID} and wait for the reply from the replica to confirm the execution result of the corresponding object. EPaxos further divides committing action into two phases. Any message committed right after the first phase is considered committed on the \textit{fast path}. Any message committed after the second phase, which includes a procedure to resolve the interference among messages, is considered committed on the \textit{slow path}. 

The fast path in EPaxos can be executed in parallel, meaning that multiple message primaries can initiate their own fast path and commit the message simultaneously, as long as none of the commands inside their messages interfere with each other. Figure \ref{fig:epaxos-fast-path} shows the fast path operated by two message primaries at the same time. In Figure \ref{fig:epaxos-fast-path}, $f = 2$ and the quorum size $f + \lfloor \frac{f+1}{2} \rfloor = 3$, therefore the quorum consist of one message primary and two other replicas for each committed message. As long as the message primary receives \msgtype{ok} message from $f$ replicas, it then directly commits the message. In EPaxos, commit messages are delivered asynchronously (the dash lines in Figure \ref{fig:epaxos-fast-path}). When two messages interfere, as shown in \ref{fig:epaxos-slow-path}, where \textit{Replica 3} detects that message from \textit{Client 1} ($R1$) depends on $R2$ from \textit{Client 2}, once the message primary (\textit{Replica 1}) receives the interfere response from \textit{Replica 1}, \textit{Replica 1} will start a second round broadcasting the dependency to quorum. When the quorum members agree on this dependency and deliver enough responses, the message primary commits the message, and all replicas will execute the message commands based on this dependency. 

\subsubsection{Consensus for message interference (execution)}

EPaxos tracks message interference by maintaining two attributes of each message $\gamma$: $deps_{\gamma}$, a list of all instances, either committed or not, that $\gamma$ depends on; and $seq_{\gamma}$, a sequence number used in execution action. When any replica sends a message $\gamma$, it always attaches the above two attributes with $\gamma$. When any replica receives $\gamma$, it will updates  $deps_{\gamma}$ unionised by all $deps_{\gamma}$ it receives plus its current instance dependency with $\gamma$, and updates $seq_{\gamma}$ to make sure  $seq_{\gamma}$ is larger than any other $seq_{\theta}$ if $\theta$ is in $deps_{\gamma}$, i.e., EPaxos makes sure that $seq_{\gamma} > seq_{\theta}$ is always true if $\gamma$ depends on $\theta$. During the execution action, EPaxos builds a dependency graph from $deps$ of executing messages, then performs a topological sort to obtain a valid execution sequence. If EPaxos detects a dependency cycle, it uses $seq$ values to break the cycle by executing the messages in ascending order of their $seq$ values.  

 
\subsubsection{ Consensus for failure recovery}

EPaxos adds an $epoch$ number into each message's ballot number to distinguish different system configurations, which results in a ballot number format as $epoch.b.R$ ($b$ for ballet number and $R$ for replica identifier). At the same time, the classic Paxos only has a simple ballot number $b.R$ for each message. 


EPaxos provides a \textit{Explicit Prepare} procedure for failure recovery. When replica $R$ fails and tries to recover an instance, it sends a \msgtype{Prepare} message with the instance's ballot number and waits for at least $\lfloor \frac{N}{2} \rfloor + 1 $ replies. The other replicas will check if the incoming \msgtype{prepare} message is worth reply, i.e., check if the received ballet number is larger than the local one. If the recovering replica receives a \msgtype{commit} message for message $\gamma$ in the recovering instance, it will run the commit phase for $\gamma$. If the recovering replica receives an \msgtype{accept} message, it will start Phase 2 of the slow path for $\gamma$. If the recovering replica receives \msgtype{pre-accepted} message(s), it may start a fast path, a slow path, or only a Phase 2 of slow path for $\gamma$, depending on the number of messages and the source of them. 

\subsubsection{ Consensus for view change: how to add a node}

EPaxos has no primary; therefore, each newly joined replica only needs to inform other nodes and learn the instances other nodes hold. EPaxos let a configuration service or human decide the new $epoch$ number, then let the replica send a \textit{Join} message and wait to receive replies, which includes committed instances, from at least $f+1$ running replicas, after which the joined replica becomes live and legit to perform the consensus. 

\subsubsection{Discussion}

EPaxos outperforms its predecessors by amortizing the primary responsibility to every replica with a geographical workload distribution. Compare to its predecessors, EPaxos achieves: (1) lower commit latency from client side because of the fast path procedure, plus the fact that a client has no need to communicate to a distant server; (2) balanced workload by its geographical distribution manner; (3) smooth performance when handling replica failure because the system can operate uninterrupted instead of suffering from a failed designated primary. EPaxos also shows more than two orders of magnitudes latency reduction under the batch mode, which majorly benefits its primary-less design. EPaxos also performs better with logs, for every replica can process its logs in parallel with other replicas. 

When the messages heavily interfere with each other, the latency of EPaxos starts to increase because it has to process the slow path and the extra message interfere procedure. However, EPaxos argues that the interference rate is fewer than $1\%$ of all commands in real industrial applications like Chubby~\cite{burrows2006chubby} and Google F1~\cite{corbett2013spanner}. Even the interfere rate is $100\%$, the latency of EPaxos only increases by 2x, and EPaxos still outperforms General-Paxos in this case. 

==> protocols/zyzzyva-shiquan.tex <==
%\newpage
\subsection{Zyzzyva: Speculative Byzantine fault tolerance}
\subsubsection{System model and service properties}

Zyzzyva~\cite{kotla2007zyzzyva, kotla2008zyzzyva, kotla2010zyzzyva} is a leader-based BFT algorithm that uses speculative executions to reduce communication costs under normal operation. Similar to PBFT~\cite{castro1999practical}, Zyzzyva has a replication protocol and a view-change protocol and tolerates $f$ Byzantine faulty replicas with $3f+1$ servers in total. 
Chiefly, instead of reaching consensus among replicas before replying to clients, Zyzzyva allows clients to collect tentative results before consensus is reached. Clients can speculatively complete a request in a fast track if all replicas reply with matching/correct execution results. 
%even though the replicas cannot learn whether the request has been completed after the speculative execution.
The speculative execution reduces message complexity from quadratic to linear in the fast track. Table \ref{tab:zyzzyva_message_table} illustrates the messaging formats in Zyzzyva.

\begin{figure*}[t]
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/zyzzyva-normal-op.pdf}
        \caption{The replication protocol of speculative executions.}
        \label{fig:zyzzyva-normal-operation}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/zyzzyva-view-change.pdf}
        \caption{The view-change protocol.}
        \label{fig:zyzzyva-view-change}
    \end{subfigure}
    \caption{The message-passing workflow of the replication and view-change protocol in Zyzzyva.}
    \label{fig:zyzzyva}
\end{figure*}

\subsubsection{The replication protocol}
Under normal operation, Zyzzyva's replication protocol operates in two phases: speculative execution and commit  (shown in Figure \ref{fig:zyzzyva-normal-operation}).
A speculative execution starts when a client sends a \textsc{request} to the primary. The client starts a timer, waiting for \textsc{spec-response} messages from replicas.
The primary then assigns a sequence number $n$ for the request and broadcasts an \textsc{order-req} message that contains a \texttt{digest} and a \texttt{history} of the request to other replicas. After receiving the \textsc{order-req} message, a replica speculatively executes the operation (\texttt{op}) in the request and directly replies with a \textsc{spec-response} message to the client with the execution result. 
At the end of this phase, if $3f+1$ responses are collected, which means the request has been correctly executed in all servers, the client adopts a fast agreement without notifying replicas. In this case, replicas are not aware of the client's decision, and thus they must preserve the sequence number and the history of executed requests until the next view change.

Moreover, if $2f+1$ responses cannot be collected before the timer expires, which suggests that the primary may have failed, the client resends the request to all replicas, and correct replicas then forward it to the primary. In addition, if some non-primary replicas are faulty, a client may receive $2f+1$ to $3f$ responses. In this case, a client starts a commit phase by setting a second timer and broadcasting a \textsc{commit} message that piggybacks a commit certificate containing all matching responses (i.e., $2f+1$ signed \textsc{spec-response} messages from different replicas). Replicas then store the certificate and send a \textsc{local commit} message to the client. If the client receives $2f+1$ \textsc{local commit} messages before its timer expires, the client completes the request. At this time, the commit certificate is stored in at least $f+1$ correct servers.
If the client fails to collect sufficient \textsc{local commit}s, it resends the request to other replicas so that a view change can be initiated when a request execution cannot be finished in time.

\subsubsection{The view-change protocol}
Since Zyzzyva introduces speculative execution to achieve fast agreements, compared with PBFT~\cite{castro1999practical}, Zyzzyva's view-change protocol is more fine-grained with a phase of no-confidence votes (Figure \ref{fig:zyzzyva-view-change}). 
A view change can be triggered in two ways: a client can \textcircled{1} disclose a \textsc{proof of misbehavior} (\textsc{POM}) targeting the primary, or \textcircled{2} complain to other replicas triggering timeouts to detect the anomaly of the primary. A \textsc{POM} message consists of a view number and a pair of \textsc{order-req} messages received by the client; the \textsc{order-req} messages have the identical view number and digest of results but different sequence numbers or history.

\input{tables/zyzzyva-message-table}

Once a replica receives a \textsc{POM} message or its timer triggers a timeout, it initiates a view change and sends out a no-confidence vote (\textsc{I-hate-the-primary} message) to other replicas. Note that in PBFT, replicas remain silence after sending out a \textsc{view-change} message, but in Zyzzyva, replicas still participate in replication in the current view during the no-confidence vote phase until they have collected enough votes for this view change. This design guarantees that potential view changes will not stop replication when a primary failure has not yet been confirmed.

When a replica receives $f+1$ no-confidence votes, it starts a view-change phase by broadcasting a \textsc{view-change} message that contains the new view number ($v+1$), the latest sequence number, $\mathcal{C}$, $\mathcal{CC}$ and $\mathcal{O}$, where $\mathcal{C}$ is the most recent commit certificate, $\mathcal{CC}$ is the proof of the last stable checkpoint including at least $2f+1$ checkpoint messages, and $\mathcal{O}$ is the history of the ordered requests after the last checkpoint. 

Next, when the new primary of view $v+1$ collects $2f+1$  \textsc{view-change} messages, it sends out a \textsc{new-view} message to all replicas, where $\mathcal{P}$ is the set of the $2f+1$ collected \textsc{view-change} messages, and $\mathcal{G}$ is the set of the history of commit certificates and ordered requests computed by the new primary based on collected \textsc{view-change} messages.

Finally, a replica broadcasts a \textsc{view-confirm} message and expects to receive $2f+1$ \textsc{view-confirm} messages (including its own) at the end of this phase. The confirmation indicates that the replica has received the \textsc{new-view} message and will operate in the next view. Note that this phase is not mandatory for guaranteeing safety; nevertheless, it indicates that all correct replicas have agreed on the history of the last view, which simplifies the safety proof.

\subsubsection{Discussion}

Zyzzyva reduces the messaging cost in replication by using speculative executions. The fast-track and two-phase design of Zyzzyva inspired many linear-cost BFT protocols, such as 700BFT~\cite{guerraoui2010next} and SBFT~\cite{gueta2019sbft}. However, the correctness of the protocol is not formally proved, and later studies show that the safety property can be violated~\cite{abraham2017revisiting}: a Byzantine primary can provide inconsistent commit certificates during different view-change phases, which lead to conflicting logs among different views.

==> tables/zyzzyva-message-table.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|r|l|}
        \hline
        Message types & Parameters piggybacked in messages\\
        \hline
        \textsc{request} & $\langle$
        \texttt{op,timestamp,clientId}
        $\rangle_{\sigma_c}$\\
        
        \textsc{order-req} & $\langle \langle$
        \texttt{view,seqNum,historyOfReq,digestOfReq,ND}
        $\rangle_{\sigma_P}$, \texttt{request}$\rangle$ \\
        
        \textsc{spec-response} & $\langle \langle$
        \texttt{view,seqNum,historyOfReq,digestOfResult,clientId,}
        \\ & \hspace{1em} \texttt{timestamp}
        $\rangle_{\sigma_i}$, \texttt{serverId,resultOfOp,order-req}
        $\rangle$ \\
        
        \textsc{commit} & $\langle$
        \texttt{clientId, commitCertificate}
        $\rangle_{\sigma_i}$\\
        
        \textsc{local-commit} & $\langle$
        \texttt{view,digestOfReq,historyOfReq,serverId,clientId}
        $\rangle_{\sigma_i}$\\
        \hline
        
        \textsc{pom} & $\langle$ 
        \texttt{view,} $\langle$ \texttt{order-req$_1$, order-req$_2$} 
        $\rangle \rangle_{\sigma_c}$\\
        \hline
        
        \textsc{i-hate-the-primary} & $\langle$ 
        \texttt{view}
        $\rangle_{\sigma_i}$ \\
        
        \textsc{view-change} & $\langle$ 
        \texttt{newView,seqNum,$\mathcal{C}$,$\mathcal{CC}$,$\mathcal{O}$,serverId}
        $\rangle_{\sigma_i}$\\
        \textsc{new-view} & $\langle$
        \texttt{newView,$\mathcal{P}$,$\mathcal{G}$}
        $\rangle_{\sigma_P}$\\
        \textsc{view-confirm} & $\langle$
        \texttt{newView,seqNum,historyOfReq,serverId}
        $\rangle_{\sigma_i}$\\
        
        \hline
    \end{tabular}
    \caption{The messaging formats in Zyzzyva.}
    \label{tab:zyzzyva_message_table}
    \vspace{-2em}
\end{table}

